Smart Resource Management for Data Streaming using an Online Bin-packing Strategy

Data stream processing frameworks provide reliable and efficient mechanisms for executing complex workflows over large datasets. A common challenge for the majority of currently available streaming frameworks is efficient utilization of resources. Most frameworks use static or semi-static settings for resource utilization that work well for established use cases but lead to marginal improvements for unseen scenarios. Another pressing issue is the efficient processing of large individual objects such as images and matrices typical for scientific datasets. HarmonicIO has proven to be a good solution for streams of relatively large individual objects, as demonstrated in a benchmark comparison with the Spark and Kafka streaming frameworks. We here present an extension of the HarmonicIO framework based on the online bin-packing algorithm, to allow for efficient utilization of resources. Based on a real world use case from large-scale microscopy pipelines, we compare results of the new system to Spark's auto-scaling mechanism.

==> inputs/harmonicio-before-ben-edit.tex <==
%HASTE\footnote{\url{http://haste.research.it.uu.se/}} (Hierarchical Analysis of Spatial and Temporal Data) is a research project that aims to provide a large-scale data stream processing platform with intelligent storage tier capabilities, appropriate for scientific image analysis applications such as electron microscopy imaging. 
One of the components of the HASTE platform is the data streaming platform HarmonicIO~\cite{hio} (HIO). HIO uses Docker containers as the processing engines (PEs) to process the streamed data; these are designed and provided by the client. The system consists of a cluster of virtual machine (VM) nodes, which can either be a master or a worker, and the PE containers are hosted on the worker nodes. Provided in Figure~\ref{fig:hio_concept} is an illustration of the platform architecture.
%The main functionality of HIO is to host containers, needed by the end user for processing data, in a cluster of virtual machines. A conceptual description of this architecture is provided in \cref{fig:hio_concept}, portraying how the system consists of a \textit{master} node, \textit{worker} nodes and the client connections via \textit{stream connectors}. The master manages the workers and the containers are hosted on worker nodes.

\begin{figure}[htbp]
    \begin{center}
    \includegraphics[width=\linewidth]{Figs/hio_concept.png}
    \end{center}
    \caption{The HarmonicIO design concept. The system consists of a master node, worker nodes and stream connectors, where solid lines indicate communication and dotted lines P2P data transfer. Image from \cite[Fig. 1]{hio}. 
    }
    \label{fig:hio_concept}
\end{figure}

To work with HIO, a user will first need to design their desired data processing task as a Docker container image and publish this to Docker Hub; examples and a template are available at the GitHub repository\footnote{https://github.com/HASTE-project/HarmonicPE}. With this in place the user can start querying a HIO server to host PEs based on this container image and the start streaming data that they wish to process. From here HIO takes care of directing the data streams to the intended PE endpoint. 

%REWRITE In a typical scenario, a user would build a Docker image that can perform some analysis on data he or she needs processed, upload this to DockerHub, and send a request to a HIO server to host a number of these containers. When these have been deployed and are running, the user can start streaming their data to the HIO master which will forward the streams to containers to process it as they were designed to.

In previous work~\cite{thesis_irm}, several changes were made to HIO in order to add support for dynamic workload scheduling and improve resource management. The main contribution was to add the possibility for the master node to autonomously decide where to host containers and remove any user-to-worker communication, making way for an algorithm that could optimize this decision. The outcome of the work was an extension of HIO adding intelligent resource management based on bin-packing, which is presented briefly in section \ref{sec:system}.

%This presents an opportunity to design and implement an extension of the platform. Thus, this project aims to design an intelligent resource management system based on bin packing for managing containers in a cluster of worker VMs, as well as actually implementing a proof of concept of this system by extending the HarmonicIO platform in order to evaluate the design. This design is fully explained in \cref{sec:system}.

%According to a comparison and benchmark by Blamey et al, \cite{blamey2018apache}
%, 
One of the strengths of HIO lies in the throughput for larger object sizes. Since one of the goals of the HASTE project is to analyze microscopy images, the target object size is much different to the typical workloads often consisting of streaming textfiles or JSON objects. Comparing HIO to similar common streaming frameworks, namely Apache Spark Streaming and Kafka, and found that HIO could achieve larger throughput for relevant object sizes.

%REWRITE With the goal of the HASTE project in mind, managing streaming of larger data objects as opposed to the common case of smaller objects becomes the focus. While several well-known and widely used streaming frameworks exist, such as Apache Spark Streaming or Kafka, these may not be optimal for this use case. In a comparison and benchmark~ between the two frameworks and HIO, \citeauthor{blamey2018apache} suggest that these popular frameworks may not be as well suited for this task. 


\subsection{Key features}
\label{subsec:hio_components}
{
\color{red}{SECTION HELP NEEDED All REWRITE paragraphs are copied from master thesis, these need rewriting and I'm not sure what to highlight from HIO - oliver}
}
% Page length   = 0.5 Page

REWRITE The reason why HIO provides an interesting alternative is that being based on \textit{peer-to-peer} (P2P) technology, it allows faster transfer of files with less CPU resources being used by the cluster for receiving the data. In turn, this leads to more available processing power.


REWRITE A brief overview of the HIO architecture is given in order to explain some features we refer to later. As mentioned, the streaming platform is based on three components~\cite{hio}, as apparent in Figure~\ref{fig:hio_concept}, which are described in the following definition list:

\begin{itemize}
\item \textbf{Master} The master node of HIO is responsible for maintaining the state of the system, keeping track of what worker nodes are connected, their availability, accepting stream requests to a stream message queue when no workers are available and starting containers, or \textit{Processing Engines} (PEs) as per user requests.
\item \textbf{Worker} The workers nodes are VMs that are connected and continuously reporting to the Master node, and can be seen as a pool or set of available streaming endpoints. The workers host PEs which contain the user-defined instructions to process data that is streamed to the PE via P2P from the stream connectors.
\item \textbf{Stream connector} The stream connector acts as the client to the HIO platform, providing a REST API for the user. The API allows requesting the address of a PE, which becomes the endpoint for the user to start streaming data to. A stream request consists of both the data to be processed, and the docker container and tag that a PE needs to run to process the data.
\end{itemize}



==> inputs/parameter_table.tex <==
\begin{table}[htbp]
    \centering
    \caption{All the parameters for the IRM system that a user can configure, along with explanations and default values. These can all be found in a JSON-formatted configuration file, read by the IRM system at startup.}
    \label{tab:parameters}
\renewcommand{\arraystretch}{2.4}
\begin{tabular}{@{}llr@{}}
\toprule[2pt]
\textbf{Parameter name}          & \textbf{Explanation}                                                                          & \parbox{0.1\linewidth}{\textbf{De\-fault value}} \\ 
%\addlinespace[0.3em] \hline
\midrule[2pt]
\texttt{packing\_interval}       & \parbox{0.3\linewidth}{\textit{Interval in seconds between performing the bin packing algorithm}}                         & $1$                      \\ \hline
\texttt{default\_cpu\_share}     & \parbox{0.3\linewidth}{\textit{Initial guess of CPU size of unencountered container images}}                          & $0.125$                  \\ \hline
\texttt{profiling\_interval}     & \parbox{0.3\linewidth}{\textit{Interval in seconds between how often worker profiler updates queued container requests}} & $4$                      \\ \hline
\texttt{predictor\_interval}     & \parbox{0.3\linewidth}{\textit{Interval in seconds between predicting load and determining scaling action}}                 & $1 $                     \\ \hline
\texttt{lower\_rate\_limit}      & \parbox{0.3\linewidth}{\textit{Lower positive threshold for load predictor}}                                          & $2$                      \\ \hline
\texttt{upper\_rate\_limit}      & \parbox{0.3\linewidth}{\textit{Upper positive threshold for load predictor}}                                          & $5$                      \\ \hline
\texttt{slowdown\_rate}          & \parbox{0.3\linewidth}{\textit{Negative threshold for load predictor}}                                                & $-2$                     \\ \hline
\texttt{queue\_size\_limit}      & \parbox{0.3\linewidth}{\textit{Message queue length limit for load predictor}}                                        & $10$                     \\ \hline
\texttt{scaleup\_waiting\_time}  & \parbox{0.3\linewidth}{\textit{Cool-down time for load predictor scaleup actions}}                                    & $10$                     \\ \hline
\texttt{large\_scaleup\_amount}  & \parbox{0.3\linewidth}{\textit{Large scaleup quantity for load predictor}}                                            & $2$                      \\ \hline
\texttt{small\_scaleup\_amount}  & \parbox{0.3\linewidth}{\textit{Small scaleup quantity for load predictor}}                                           & $1$                      \\ \hline
\texttt{container\_request\_TTL} & \parbox{0.3\linewidth}{\textit{Initial time-to-live counter for container requests}}                                     & $1$ \\
\bottomrule[2pt]
\end{tabular}

\end{table}
